WIYN Open Cluster Study. XXIV. Stellar Radial-Velocity Measurements in NGC 6819

We present the current results from our ongoing radial-velocity survey of the intermediate-age (2.4 Gyr) open cluster NGC 6819. Using both newly observed and other available photometry and astrometry we define a primary target sample of 1454 stars that includes main-sequence, subgiant, giant, and blue straggler stars, spanning a magnitude range of 11<=V<=16.5 and an approximate mass range of 1.1 to 1.6 Msun. Our sample covers a 23 arcminute (13 pc) square field of view centered on the cluster. We have measured 6571 radial velocities for an unbiased sample of 1207 stars in the direction of the open cluster NGC 6819, with a single-measurement precision of 0.4 km/s for most narrow-lined stars. We use our radial-velocity data to calculate membership probabilities for stars with >= 3 measurements, providing the first comprehensive membership study of the cluster core that includes stars from the giant branch through the upper main sequence. We identify 480 cluster members. Additionally, we identify velocity-variable systems, all of which are likely hard binaries that dynamically power the cluster. Using our single cluster members, we find a cluster average radial velocity of 2.34 +/- 0.05 km/s . We use our kinematic cluster members to construct a cleaned color- magnitude diagram from which we identify rich giant, subgiant, and blue straggler populations and a well-defined red clump. The cluster displays a morphology near the cluster turnoff clearly indicative of core convective overshoot. Finally, we discuss a few stars of note, one of which is a short-period red-clump binary that we suggest may be the product of a dynamical encounter.

==> tab4.tex <==
\begin{deluxetable}{cc}
\tablewidth{0pc} 
\tablecolumns{2}
\tablecaption{
The number of stars with WOCS radial-velocity measurements in each
membership and binarity category, as discussed in the text.
\label{t:cat}}
\tablehead{
\colhead{Category } &
\colhead{Number of Stars } 
}
\startdata
SM & \numcatSM \\
SN & \numcatSN \\
BM & \numcatBM \\
BN & \numcatBN \\
BLM & \numcatBLM \\
BLN & \numcatBLN \\
BU & \numcatBU \\
U & \numcatU \\
\enddata
\end{deluxetable}

